ORACLE: Collaboration of Data and Control Planes to Detect DDoS Attacks

The possibility of programming the control and data planes, enabled by the Software-Defined Networking (SDN) paradigm, represents a fertile ground on top of which novel operation and management mechanisms can be fully explored, being Distributed Denial of Service (DDoS) attack detection based on machine learning techniques the focus of this work. To carry out the detection, this paper proposes ORACLE: cOllaboRation of dAta and Control pLanEs to detect DDoS attacks, an architecture that promotes the coordination of control and data planes to detect network attacks. As its first contribution, this architecture delegates to the data plane the extraction and processing of traffic information collected per flow. This is done in order to ease the calculation and classification of the feature set used in the attack detection, as the needed flow information is already processed when it arrives at the control plane. Besides, as the second contribution, this architecture breaks the limitations to calculate some features that are not possible to implement in a traditional OpenFlow-based environment. In the evaluation of ORACLE, we obtained up to 96% of accuracy in the testing phase, using a K-Nearest Neighbor model.

==> ControlPlane.tex <==
\section{Implementation at the Control Plane}
How was said in section III, the control plane has the responsibility to calculate the features with the statistics sent by the data plane and make the classification in search of DDoS attacks. To receive these statistics at the control plane, we developed an application in the controller that can receive the control packets and extract each custom header field. Then each field is parsed to get the set of statistics of each flow. This set of statistics is listed in table \ref{tabla:statistics}. This set contains the first feature and the needed information pre-processed to calculate the other features with less effort.

In table \ref{tabla:features} we can see that F2, F3, and F4 are based on average (avg) and standard deviations (std) operations. To calculate those features we use the equations \ref{eq:mean} and \ref{eq:std}. The traditional equation \ref{eq:std} was transformed in the representation of the right side using arithmetic properties because otherwise, we would need the individual information of each packet ($x_{i}$) to calculate the std, method little efficient that wastes storage resources and execution time. With the new representation is not necessary to have all the ($x_{i}$), instead of that, we can program the data plane to send into the set of statistics the results of the summations $\sum x_{i}$ and $\sum x_{i}^{2}$, Hence, the calculation of the std would be simply replacing values into the equation and make simple arithmetic operations. 

\begin{equation}\label{eq:mean}
    \overline{x} = \frac{\sum_{i:1}^{n} x_{i}}{n - 1}
\end{equation}

\begin{equation}\label{eq:std}
    std = \sqrt{\frac{\sum_{i:1}^{n}\left ( x_{i} - \overline{x} \right )^{2}}{n-1}} = \sqrt{\frac{\sum_{i:1}^{n}x_{i}^{2}-2\overline{x}\sum_{i:1}^{n}x_{i}+n\overline{x}^{2}}{n-1}}
\end{equation}

On the other hand, the classifier was implemented into the same control plane but out from the controller. This has a web service implemented with the \textit{Bottle} library of python, who allows receiving tuples with the features. The classifier loads an ML model previously trained together with its parameters of standardization of the data. The models' explanation loaded is at the session VI. 

%How was said in section III, the control plane has the responsibility to calculate the features that were not possible to calculate at the data plane and send all of them to the classifier. The set of features selected to detect the DDoS attack is specified in the Table \ref{tabla:features} which is formed with features based on time, bytes and behavior. In \cite{CICIDS2017} is demonstrated that this set of features are the best descriptors of the DDoS attack between a big quantity of features specified in the CICIDS-2017 dataset that is detailed in section VI. In the last column of the table, we can see that the last three features are calculated in the control plane because P4 does not support division operation that is necessary to calculate averages (avg) and standard deviations (std).

%To calculate the avg and std of the set of data X with size n, we use the equation \ref{eq:mean} and \ref{eq:std} respectively. The traditional equation \ref{eq:std} was transformed using arithmetic properties in the representation of the right side due to the traditional way would require that the Data Plane sends the set of values X to calculate each subtraction of squares, thing that would demand more storage at the data plane and more time execution spent at the control plane. With the new representation is not necessary have the set of values X due to is easier by the system that the data plane sends directly the equation summations results simplifying the work and the resources in both planes. All these statistics per flow sent are listed in the table \ref{tabla:statistics}.  We can verify that the values of the summation of $x_{i}^{2}$ are provided by S6 and S8, the values of the summation of $x_{i}$ are provide by S4, S5 and S7, and $n$ by S2 and S3, depending of the features to calculate. To implement this, we developed an application in the controller that can receive the packets\_in and only filter the packets with flow statistics. When these packets arrived to the controller, the custom header is extracted and each header field is parsed getting the statistics of each flow sent.  

\begin{table}[]
  \begin{center}
    \caption{Statistics per Flow Sent by the Data Plane}
    \label{tabla:statistics}
    \resizebox{9cm}{!}{
    \begin{tabular}{c|l|l}
      \toprule % <-- Toprule here
      \textbf{\#} & \textbf{Statistic} & \textbf{Description} \\
      \midrule % <-- Midrule here
                    F1 & Feduration & Flow duration in microseconds      \\
                    \hline
                    S2 & Tot Fwd Pkt & Total number of packets in the forward direction                \\ 
                    \hline
                    S3 & Tot Bwd pkt & Total number of packets in the backward direction               \\
                    \hline
                    S4 & Tot Len Fwd Pkt & Sum of packets size in forward direction          \\
                    \hline
                    S5 & Tot Len Bwd Pkt & Sum of packets size in backward direction         \\
                    \hline
                    S6 & Tot Len Bwd Pkt Sqrt & Sum of the square of packets size in forward direction \\
                    \hline
                    S7 & IAT Total & Sum of the packets inter arrival time \\
                    \hline
                    S8 & IAT Total Sqrt & Sum of the square of packets inter arrival time\\
                    
      \bottomrule 
    \end{tabular}}
  \end{center}
\end{table}

%\subsection{The Classifier}
%The classifier was implemented into the same control plane but out from the controller. This is a web services developed with the \textit{Bottle} library in python who is waiting for a tuples with the values of the four features to be classified the flow into Benign or DDoS. The classifier load a ML model previously trained together with its parameters of standardization of the data.\\
%The model chosen for training is the \textit{Random Forest (RF)} who is suitable for large datasets how is our case and also because is highly robust to noisy data. The random forest is an ensemble learning method who works with a multitude of decision trees to decide through the vote which is the class to belong the sample \cite{RF-Doc}. In the table \ref{tabla:training} we can see the result of the accuracy changing the maximum depth of the trees. the three cases were trained with 500 trees into the forest and 70\% of the dataset. With the remaining 30\% was validated and tested the model. From the table we can see that while the maximum depth is increased, the accuracy too. We chosen the model with $0,933$ of accuracy to test the architecture instead the model with $0,993$ because this tend to be overfitting.

%\begin{table}[]
%  \begin{center}
%    \caption{Model Training Results}
%    \label{tabla:training}
%    \begin{tabular}{c|c|c}
%      \toprule % <-- Toprule here
%      \textbf{Model} & \textbf{Parameters} & \textbf{Accuracy} \\
%      \midrule % <-- Midrule here
%\multirow{3}{*}{RF} & n\_estimators=500, max\_depth=2 & 0.923      
%\\
%                        & n\_estimators=500, max\_depth=3 & 0.933                      %\\
%                        & n\_estimators=500, max\_depth=4 & 0.993                             \\ 
%      \bottomrule % <-- Bottomrule here
%    \end{tabular}
%  \end{center}
%\end{table}

==> DataPlane.tex <==
\section{Implementation at the Data Plane}
The most important entity used at the data plane is the \textit{Register}. It is an extern object of P4 that allows creating arrays of fixed size into the switch, with operations of reading and writing available for each cell \cite{tracking}. 

To access and modify each cell of the register in an efficient manner, we implemented a data structure based on hash tables to have more performance to handle the registers in line rate. This data structure consists of using a function hash to map the flow identifier of each packet (key)  to a position into the register (index) where the statistics belonging to this flow are stored. 

Ideally, the hash function will assign each key to a unique index of the register. In the practice, depending on the range of values that the hash function can return, we might have high or low hash collisions probability, that is mean, the hash function would generate the same index for more than one key.  The range of value of the hash function is directly proportionate to the size of the register, for this reason is very important to define the correct size of the registers to have a low collision probability. With the equation (\ref{eq:fp}) is possible to estimate the collision probability where M is the number of cells into the register and N is the number of possible flow identifiers that we could have \cite{bloomfilter}.

\begin{equation}\label{eq:fp}
    C = 1 - \left ( 1 - \frac{1}{M} \right )^{N}
\end{equation}

%\subsection{Module Statistics Collector}


\subsection{Module Handler of Time and Registers}
This module defines time windows of t-seconds. In each window, the system must be able to collect new flow statistics and at the same time, send to the controller the statistics collected in the previous time window. The principal challenge implementing both tasks in parallel is not to confuse between the indexes stored into the control registers belongs to the previous time window, with the indexes stored in the current time window. 

To overcome this challenge, we thought in something similar to a road with two carriageways where each one has its own control registers working independently. See in Fig.\ref{fig:HandlerModule}. At the beginning of each time window, this module always will have the control registers empties in one of the side of the road, and on the other side, the control registers filled ready to be emptied sending to the controller the flow statistics collected in the previous time window. According to this approach, we are avoiding confusions with the indexes stored in each time window.

In Fig.\ref{fig:HandlerModule} we can see a system working with a time window of 20 seconds. Each change of window this module change the task between carriageways of the road. For instance, in the third time window, the statistics collector module is storing the new flow statistic indexes into the control registers of the right side, and in the left side, the statistic sender module is sending the flow statistics stored in the control registers of this side.

On the other hand, besides of handling the time windows, this module has the responsibility to validate in each time window if there are flow statistics to still send to the controller. in case there are still flows, this module use a primitive of P4 to clone the packet that arrived and send it to the sender statistics module with the statistics of the flows to send.

\begin{figure}[] 
    \centering
    \includegraphics[scale=0.5]{Figures/handlermodule.pdf}
    \caption{Road with 2 carriageways: The Mechanism to handle the time windows}
    \label{fig:HandlerModule}
\end{figure}

\subsection{Module Statistics Sender}
This module was designed to send in a compact manner 10, 5 or 1 flow per control packet, where the priority is always to send 10 flows as long as the quantity is available. Sending various flow statistics in an only packet helps to reduce the number of packets injected to the network and the total time needed to send the information of all flows collected into a time window.

\begin{figure}[] 
    \centering
    \includegraphics[scale=0.55]{Figures/headers.pdf}
    \caption{Control packet that contains the flow statistics.}
    \label{fig:PacketCloned}
\end{figure}

This module receives the packet cloned from the handler module in a different thread together with the statistics of the set of flow to be sent.  After that, the packet cloned is transformed into a control packet how is depicted in  Fig.\ref{fig:PacketCloned}. The headers not necessary like IP, TCP or UDP are removed. Instead of that,  the packet is built again with a Packet\_In header,  the Ethernet header is conserved and a custom header which has the statistics of each flow. The module uses 3 different custom headers depending on the number of flows to sent. Each field (FlowX) of the custom header will carry the concatenation in bits of the statistics of one flow, furthermore of a control field that will inform the controller how many flows contain the control packet. In the end, the module forwards the original packet to its destination and the control packet toward the control plane.


==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************

